Online Lewis Weight Sampling

The seminal work of Cohen and Peng introduced Lewis weight sampling to the theoretical computer science community, yielding fast row sampling algorithms for approximating $d$-dimensional subspaces of $\ell_p$ up to $(1+\epsilon)$ error. Several works have extended this important primitive to other settings, including the online coreset and sliding window models. However, these results are only for $p\in\{1,2\}$, and results for $p=1$ require a suboptimal $\tilde O(d^2/\epsilon^2)$ samples. In this work, we design the first nearly optimal $\ell_p$ subspace embeddings for all $p\in(0,\infty)$ in the online coreset and sliding window models. In both models, our algorithms store $\tilde O(d^{1\lor(p/2)}/\epsilon^2)$ rows. This answers a substantial generalization of the main open question of [BDMMUWZ2020], and gives the first results for all $p\notin\{1,2\}$. Towards our result, we give the first analysis of "one-shot'' Lewis weight sampling of sampling rows proportionally to their Lewis weights, with sample complexity $\tilde O(d^{p/2}/\epsilon^2)$ for $p>2$. Previously, this scheme was only known to have sample complexity $\tilde O(d^{p/2}/\epsilon^5)$, whereas $\tilde O(d^{p/2}/\epsilon^2)$ is known if a more sophisticated recursive sampling is used. The recursive sampling cannot be implemented online, thus necessitating an analysis of one-shot Lewis weight sampling. Our analysis uses a novel connection to online numerical linear algebra. As an application, we obtain the first one-pass streaming coreset algorithms for $(1+\epsilon)$ approximation of important generalized linear models, such as logistic regression and $p$-probit regression. Our upper bounds are parameterized by a complexity parameter $\mu$ introduced by [MSSW2018], and we show the first lower bounds showing that a linear dependence on $\mu$ is necessary.

==> deterministic-lewis-weight-estimation.tex <==
\section{Deterministic Online Lewis Weight Estimation}\label{sec:det-lewis}


The following is the deterministic \textsc{OnlineBSS} algorithm of \cite{BDMMUWZ2020}, which derandomizes an algorithm of \cite{CMP2020} with only logarithmic overheads.

\begin{Theorem}[Deterministic \textsc{OnlineBSS}, Appendix B.2, \cite{BDMMUWZ2020}]\label{thm:det-online-bss}
Let $\bfA\in\mathbb R^{n\times d}$. Let $\eps\in(0,1)$ be an accuracy parameter. Then, there is a deterministic online coreset algorithm \textsc{DetOnlineBSS} which stores a weighted subset $\tilde\bfA$ of $m$ rows for
\[
    m = O\parens*{\frac{d}{\eps^2}(\log n)(\log\kappa(\bfA))}
\]
such that
\[
    (1-\eps)\tilde\bfA_i^\top\tilde\bfA_i \preceq \bfA_i^\top\bfA_i \preceq (1+\eps)\tilde\bfA_i^\top\tilde\bfA_i
\]
for all $i\in[n]$.
\end{Theorem}

Using this primitive, we give Algorithm \ref{alg:det-online-lewis-weight-estimate}, which is a deterministic algorithm for estimating weights $\tilde\bfw_i$. 

\begin{algorithm}
	\caption{Deterministic Online Lewis Weight Estimation}
	\textbf{input:} $\bfA\in\mathbb R^{n\times d}$, $p\in(0,\infty)$. \\
	\textbf{output:} Online Lewis weight estimates $\braces*{\tilde\bfw_i}_{i=1}^n$.
	\begin{algorithmic}[1] %
        \State Initialize \textsc{DetOnlineBSS} with $\eps=1/2$ (Theorem \ref{thm:det-online-bss})
        \For{$i\in[n]$}
            \If{$\rank(\bfA_i) > \rank(\bfA_{i-1})$}
                \State $\tilde\bfw_i \gets 1$
            \Else
                \State Let $\tilde \bfM_{i-1}$ be the approximate quadratic form provided by \textsc{DetOnlineBSS}\label{line:bss-est}
                \State $\tilde\bfw_i \gets \min\braces*{[2\cdot\bfa_i^\top\tilde\bfM_{i-1}^-\bfa_i]^{p/2}, 1}$
            \EndIf
            \State Update \textsc{DetOnlineBSS} with the row $\tilde\bfw_i^{1/2-1/p}\bfa_i$
        \EndFor
        \State \Return $\braces*{\tilde\bfw_i}_{i=1}^n$
	\end{algorithmic}\label{alg:det-online-lewis-weight-estimate}
\end{algorithm}

We first show that the weights generated by Algorithm \ref{alg:det-online-lewis-weight-estimate} are one-sided $\ell_p$ Lewis weights.

\begin{Lemma}\label{lem:lw-ls-b}
Let $\bfA\in\mathbb R^{n\times d}$ and let $0<p<\infty$. Let $\tilde\bfw_i$ be weights generated by Algorithm \ref{alg:det-online-lewis-weight-estimate}, and let $\tilde\bfW = \diag(\tilde\bfw)$. Then, for all $i\in[n]$,
\[
    \tilde\bfw_i \geq \bftau_i\parens*{\tilde\bfW^{1/2-1/p}\bfA}.
\]
\end{Lemma}
\begin{proof}
If $\tilde\bfw_i \geq 1$, then we already have the claim since leverage scores are always at most $1$, so assume that $\tilde\bfw_i < 1$. In particular, we have that $\bfa_i\in\rowspan(\bfA_{i-1})$. Then, with $\tilde\bfM_{i-1}$ defined as in Line \ref{line:bss-est},
\[
    \tilde\bfM_{i-1} \preceq \frac32 \tilde\bfA_{i-1}^\top\tilde\bfW_{i-1}^{1-2/p}\tilde\bfA_{i-1}
\]
by the deterministic guarantee of \textsc{DetOnlineBSS}. Then by Lemma \ref{lem:psd-flip}, 
\[
    \tilde\bfw_i^{2/p} = 2\cdot \bfa_i^\top\tilde\bfM_{i-1}^-\bfa_i \geq 2\cdot \frac23 \bfa_i^\top(\tilde\bfA_{i-1}^\top\tilde\bfW_{i-1}^{1-2/p}\tilde\bfA_{i-1})^-\bfa_i > \bfa_i^\top(\tilde\bfA_{i-1}^\top\tilde\bfW_{i-1}^{1-2/p}\tilde\bfA_{i-1})^-\bfa_i
\]
so
\[
    \tilde\bfw_i \geq (\tilde\bfw_i^{1/2-1/p}\bfa_i)^\top(\bfA_{i-1}^\top\tilde\bfW_{i-1}^{1-2/p}\bfA_{i-1})^-(\tilde\bfw_i^{1/2-1/p}\bfa_i) = \bftau_i^{\OL}(\tilde\bfW^{1/2-1/p}\bfA) \geq \bftau_i(\tilde\bfW^{1/2-1/p}\bfA),
\]
which is the desired statement.
\end{proof}

Next, we show that these weights have a small sum. For this, we first show that these weights are bounded by the online leverage scores of a reweighted matrix:

\begin{Lemma}
    Let $\bfA\in\mathbb R^{n\times d}$ and $0<p<\infty$. Let $\tilde\bfw_i$ be weights generated by Algorithm \ref{alg:det-online-lewis-weight-estimate}, and let $\tilde\bfW = \diag(\tilde\bfw)$. Then,
    \[
        \tilde\bfw_i \leq 4\cdot\bftau_i^\OL(\tilde\bfW^{1/2-1/p}\bfA)
    \]
\end{Lemma}
\begin{proof}
We have equality for $\bfa_i \notin \rowspan(\bfA_{i-1})$, with both being $1$. It remains to bound the $\tilde\bfw_i$ for $\bfa_i \in \rowspan(\bfA_{i-1})$. Then, with $\tilde\bfM_{i-1}$ defined as in Line \ref{line:bss-est},
\[
    \tilde\bfM_{i-1} \succeq \frac12 \tilde\bfA_{i-1}^\top\tilde\bfW_{i-1}^{1-2/p}\tilde\bfA_{i-1}
\]
by the deterministic guarantee of \textsc{DetOnlineBSS}. Then by Lemma \ref{lem:psd-flip}, 
\[
    \tilde\bfw_i^{2/p} \leq 2\cdot \bfa_i^\top\tilde\bfM_{i-1}^-\bfa_i \leq 2\cdot 2\cdot \bfa_i^\top(\tilde\bfA_{i-1}^\top\tilde\bfW_{i-1}^{1-2/p}\tilde\bfA_{i-1})^-\bfa_i = 4\cdot \bfa_i^\top(\tilde\bfA_{i-1}^\top\tilde\bfW_{i-1}^{1-2/p}\tilde\bfA_{i-1})^-\bfa_i
\]
so
\[
    \tilde\bfw_i \leq 4\cdot(\tilde\bfw_i^{1/2-1/p}\bfa_i)^\top(\bfA_{i-1}^\top\tilde\bfW_{i-1}^{1-2/p}\bfA_{i-1})^-(\tilde\bfw_i^{1/2-1/p}\bfa_i) = 4\cdot \bftau_i^{\OL}(\tilde\bfW^{1/2-1/p}\bfA).
\]
\end{proof}

It remains to bound the sum of the online leverage scores of $\tilde\bfW^{1/2-1/p}\bfA$, which involves bounding the condition number of $\tilde\bfW^{1/2-1/p}\bfA$. For $p>2$, this is related to the condition number of $\bfA$ up to a $\poly(n)$ factor by Lemmas \ref{lem:oslw-sensitivity} and \ref{lem:lp-overestimate}. For $0<p<2$, we directly compare $\tilde\bfw_i$ to the true $\ell_p$ Lewis weights in order to bound the condition number to within a $\poly(n)$ factor of the condition number of $\bfA$.

\begin{Lemma}\label{lem:lw-analogue-bound-0<p<2}
    Let $\bfA\in\mathbb R^{n\times d}$ and $0<p<2$. Let $\tilde\bfw_i$ be weights generated by Algorithm \ref{alg:det-online-lewis-weight-estimate}, and let $\tilde\bfW = \diag(\tilde\bfw)$. Then, for all $i\in[n]$,
    \[
        \bfw_i^p(\bfA) \leq \tilde\bfw_i.
    \]
    Furthermore, for all $\bfx\in\mathbb R^d$,
    \[
        \norm*{\bfA\bfx}_2 \leq \norm*{\tilde\bfW^{1/2-1/p}\bfA\bfx}_2 \leq d^{1/p-1/2}\norm*{\bfA\bfx}_p.
    \]
\end{Lemma}
\begin{proof}
By an inductive proof almost identical to that of Lemma \ref{lem:lw-ls-b}, we have that
\[
    \bfw_i^p(\bfA) \leq \tilde\bfw_i
\]
for every $i\in[n]$. Then, since $1-2/p<0$ for $p\in(0,2)$, we have
\[
    \norm*{\tilde\bfW^{1-2/p}\bfA\bfx}_2 \leq \norm*{\bfW^p(\bfA)^{1-2/p}\bfA\bfx}_2 \leq d^{1/p-1/2}\norm*{\bfA\bfx}_p
\]
and
\[
    \norm*{\tilde\bfW^{1-2/p}\bfA\bfx}_2 \geq \norm*{\bfA\bfx}_2.\qedhere
\]
\end{proof}

We thus have
\[
    \norm*{(\tilde\bfW_i^{1/2-1/p}\bfA_i)^-}_2 \leq \poly(n)\norm*{\bfA_i^-}_2,
\]
for every $i\in[n]$, which results in the following sum of approximate online Lewis weights:

\begin{Lemma}\label{lem:det-olw}
Let $p\in(0,\infty)$ and $\bfA\in\mathbb R^{n\times d}$. Let $\tilde\bfw\in\mathbb R^n$ be generated from Algorithm \ref{alg:det-online-lewis-weight-estimate}. Then,
\[
    \sum_{i=1}^n \tilde\bfw_i \leq O(d)\log(n\kappa^\OL(\bfA)).
\]
\end{Lemma}
\begin{proof}
We have that
\begin{align*}
    \sum_{i=1}^n \tilde\bfw_i &\leq \sum_{i=1}^n 4\cdot \bftau_i^\OL(\tilde\bfW^{1/2-1/p}\bfA) \\
    &\leq O(d)\log\kappa^\OL(\tilde\bfW^{1/2-1/p}\bfA) \\
    &\leq O(d)\log(n\kappa^\OL(\bfA)).\qedhere
\end{align*}
\end{proof}

As a result, of our Lewis weight estimates as well as our new one-shot Lewis weight sampling result of Theorem \ref{thm:one-shot-lewis-weight-sampling} for $p>2$ or Theorem \ref{thm:lewis-weight-sampling-0<p<2} for $p<2$, we obtain our main online sampling result:

\begin{Theorem}\label{thm:online-lewis-p>2}
    Let $\bfA\in\mathbb R^{n\times d}$ and $p\in(0,\infty)$. Let $\delta\in(0,1)$ be a failure rate parameter and let $\eps\in(0,1)$ be an accuracy parameter. Then there is an online coreset algorithm $\mathcal A$ such that, with probability at least $1-\delta$, $\mathcal A$ outputs a weighted subset of $m$ rows with sampling matrix $\bfS$ such that
    \[
        \norm*{\bfS_i\bfA_i\bfx}_p^p = (1\pm\eps)\norm*{\bfA_i\bfx}_p^p
    \]
    for all $\bfx\in\mathbb R^d$, for every $i\in[n]$, and
    \[
        m = \begin{dcases}
            O\parens*{\frac{d^{p/2}}{\eps^2}}(\log(n\kappa^\OL))^{p/2+1}\bracks*{(\log d)^2(\log n) + \log\frac1\delta} & p\in(2,\infty) \\
            O\parens*{\frac{d}{\eps^2}}\log(n\kappa^\OL)\bracks*{(\log d)^2\log n + \log\frac1\delta} & p \in (1,2) \\
            O\parens*{\frac{d}{\eps^2}}\log(n\kappa^\OL)\log\frac{n}{\delta} & p = 1 \\
            O\parens*{\frac{d}{\eps^2}}\log(n\kappa^\OL)\bracks*{(\log d)^3 + \log\frac1\delta} & p\in(0,1)
        \end{dcases}
    \]
\end{Theorem}



==> graveyard.tex <==



We first precondition the matrix in input sparsity time so that the condition number is O(1). Now suppose we sample each row with probability $d^{p/2-1} w_i^{p, OL}(A) / \epsilon^2$. By symmetrization, the expected error of the subspace embedding is then
$$
\mathbb E_\sigma \left[\left|\sum_{i=1}^n \sigma_i \left|\langle s_i a_i, x\rangle\right|^p\right|\right]
$$
where $s_i$ is set to $1/p_i$ with probability $p_i = d^{p/2-1} w_i^{p, OL}(A) / \epsilon^2$. Let this sketch be $SA$. We then define $A''$, which is the vertical concatenation of $A'$ and $SA$ with $A'$ on top, where $A'$ is a split up version of $A$ so that all online Lewis weights are at most $\epsilon^2/d^{p/2-1}$. Then, the above expectation is bounded by
$$
\mathbb E_\sigma \left[\left|\sum_{i=1}^n \sigma_i \left|\langle a''_i, x\rangle\right|^p\right|\right]
$$
We now claim that $A''$ has online Lewis weights bounded by $\epsilon^2/d^{p/2-1}$. This is clearly true for all rows of $A'$ in $A''$, so consider row $j$ of $A''$ that comes from $SA$. Let $i$ be the corresponding index of this row when it belongs to $A$, and let $k$ be the index of this row as the first of its copies in the split version $A'$. 
Then,
\begin{align*}
w_j^{p,OL}(A'')^{2/p} &\leq (s_i a_i)^\top (A_{j-1}'' W^{p,OL}(A'')_{j-1}^{1-2/p}A_{j-1}'')^- (s_ia_i) \\
&\leq (s_i a_i)^\top (A_{k-1}' W^{p,OL}(A')_{k-1}^{1-2/p}A_{k-1}')^- (s_ia_i) \\
&\leq (s_i a_i)^\top (A_{i-1} W^{p,OL}(A)_{i-1}^{1-2/p}A_{i-1})^- (s_ia_i) \\
&= \frac{w_i^{p,OL}(A)\epsilon^2}{w_i^{p,OL}(A)\cdot d^{p/2-1}} = \frac{\epsilon^2}{d^{p/2-1}}
\end{align*}
We can then apply the result of Ledoux-Talagrand on $A''$ to conclude.




We show a slight variation on this result, which is a sharper version of the sensitivity bound above.

\begin{Lemma}\label{lem:sharp-one-sided-sensitivity-bound}
    Let $\bfA\in\mathbb R^{n\times d}$ and $p\in(0,\infty)$. Let $\bfw$ be one-sided $\ell_p$ Lewis weights for $\bfA$ and let $\bfR$ be a one-sided $\ell_p$ Lewis basis. Then, for every $i\in[n]$, 
    \[
        \sup_{\bfx\in\rowspan(\bfA)\setminus\{0\}} \frac{\abs*{\angle*{\bfa_i,\bfx}}^p}{\norm*{\bfA\bfx}_p^p} \leq \norm*{\bfw}_1^{0\lor(p/2-1)}\bftau_i(\bfW^{1/2-1/p}\bfA)^{p/2}\bfw_i^{1-p/2}
    \]
\end{Lemma}
\begin{proof}
    The proof of Lemma 2.10 of \cite{WY2022} shows that
    \[
        \norm*{\bfx}_2^2 \leq \norm*{\bfw}_1^{1-2/p}\norm*{\bfA\bfR\bfx}_p^2.
    \]
    Furthermore, the proof of Lemma 2.8 of \cite{WY2022} shows that
    \[
        \bftau_i(\bfW^{1/2-1/p}\bfA) = \bfw_i^{1-2/p}\norm*{\bfe_i^\top\bfA\bfR}_2^2
    \]
    Then,
    \begin{align*}
        \frac{\abs*{[\bfA\bfR\bfx](i)}^p}{\norm*{\bfA\bfR\bfx}_p^p} &\leq \frac{\norm*{\bfe_i^\top\bfA\bfR}_2^p\norm*{\bfx}_2^p}{\norm*{\bfA\bfR\bfx}_p^p} \leq \bftau_i(\bfW^{1/2-1/p}\bfA)^{p/2}\bfw_i^{1-p/2}\frac{\norm*{\bfA\bfR\bfx}_p^p}{\norm*{\bfA\bfR\bfx}_p^p} = \bftau_i(\bfW^{1/2-1/p}\bfA)^{p/2}\bfw_i^{1-p/2}.
    \end{align*}
\end{proof}
